Mixin Composition Synthesis based on Intersection Types

We present a method for synthesizing compositions of mixins using type inhabitation in intersection types. First, recursively defined classes and mixins, which are functions over classes, are expressed as terms in a lambda calculus with records. Intersection types with records and record-merge are used to assign meaningful types to these terms without resorting to recursive types. Second, typed terms are translated to a repository of typed combinators. We show a relation between record types with record-merge and intersection types with constructors. This relation is used to prove soundness and partial completeness of the translation with respect to mixin composition synthesis. Furthermore, we demonstrate how a translated repository and goal type can be used as input to an existing framework for composition synthesis in bounded combinatory logic via type inhabitation. The computed result is a class typed by the goal type and generated by a mixin composition applied to an existing class.

==> IntTheory.tex <==
%!TEX root = main_document.tex

\newpage

%\begin{defi}[Type inclusion: record types]\label{def:typeInclusionRec-new}
%~ \hfill
%\begin{enumerate}
%\item \label{leq-ax-1} $\record{l:\sigma} \leq \record{}$
%\item \label{leq-ax-2} $\Pair{l:\sigma}\inter\Pair{l:\tau} \leq \Pair{l:\sigma\inter\tau}$
%\item \label{leq-ax-3} $\sigma \leq \tau \Then \Pair{l:\sigma} \leq \Pair{l:\tau}$
%\item \label{leq-ax-4} $\rho + \record{} = \record{} + \rho = \rho$
%\item \label{leq-ax-5} $(\rho_1 + \rho_2) + \rho_3 = \rho_1 + (\rho_2 + \rho_3)$
%\item \label{leq-ax-6} $(\rho_1 \inter \rho_2) + \rho_3 = (\rho_1 + \rho_3) \inter (\rho_2 + \rho_3)$
%% \item \label{leq-ax-7} $\Pair{l:\sigma} + \Pair{l:\tau} =  \Pair{l:\tau}$
%\item \label{leq-ax-8} $\Pair{l:\sigma} + (\Pair{l:\tau} \inter \rho) = \Pair{l:\tau} \inter \rho$
%%\item \label{leq-ax-9} $\Pair{l:\sigma} + \Pair{l':\tau} =  \Pair{l:\sigma} \inter \Pair{l':\tau}$ if $l\neq l'$
%\item \label{leq-ax-10} $\Pair{l:\sigma} + (\Pair{l':\tau} \inter \rho) = \Pair{l':\tau} \inter (\Pair{l:\sigma} + \rho)$ 
%				if  $l\neq l'$
%\item \label{leq-ax-11} $\rho_1 \leq \rho_2 \Then \rho_1 + \rho \leq \rho_2 + \rho$
%\item \label{leq-ax-12} $\rho_1 = \rho_2 \Then \rho + \rho_1 = \rho + \rho_2$
%\end{enumerate}
%\end{defi}

We show below some derivable through useful and natural properties of $\leq$ and $=$.

\begin{lem}\label{lem:derivedLeq-1}
~ \hfil
\begin{enumerate}
\item \label{lem:derivedLeq-1-a} $\Pair{l:\sigma}\inter\Pair{l:\tau} = \Pair{l:\sigma\inter\tau}$
\item 
\end{enumerate}
\end{lem}

\begin{lem}\label{lem:congruence}
~\hfill
\begin{enumerate}
\item \label{lem:congruence-a} 
	$\sigma_1 \leq \tau_1 \And \sigma_2 \leq \tau_2 \Then 
			\sigma_1 \inter \sigma_2 \leq \tau_1 \inter \tau_2$,
\item \label{lem:congruence-b} 
	$\rho_1 = \rho_1' \And \rho_2 = \rho_2' \Then \rho_1 \inter \rho_2 \leq \rho_1' \inter \rho_2'$,
\item \label{lem:congruence-c} 
	$\rho_1 = \rho_1' \And \rho_2 = \rho_2' \Then \rho_1 + \rho_2 \leq \rho_1' + \rho_2'$.
\end{enumerate}
\end{lem}

\begin{proof}
~\hfill
\begin{enumerate}
\item 
\item By the hypothesis and transitivity we have $\sigma_1 \inter \sigma_2 \leq \sigma_1 \leq \tau_1$
	and $\sigma_1 \inter \sigma_2 \leq \sigma_2 \leq \tau_2$ from which
	$\sigma_1 \inter \sigma_2 \leq \tau_1 \inter \tau_2$ follows by Definition \ref{def:typeInclusionInt}.
\item Immediate from (\ref{lem:congruence-a}) and the definition of $=$.
\item By \ref{def:typeInclusionRec-new}.\ref{leq-ax-11} and the definition of $=$ we have
	\[ \rho_1 = \rho_1'  \Then \rho_1 + \rho_2 \leq \rho_1' + \rho_2 \]
	By \ref{def:typeInclusionRec-new}.\ref{leq-ax-12} we have
	\[ \rho_2 = \rho_2'  \Then \rho_1' + \rho_2 \leq \rho_1' + \rho_2' \]
	hence the thesis by transitivity.
\end{enumerate}

\end{proof}


\medskip
\noindent
Abbreviation $\Pair{l_i:\sigma_i \mid i\in I \neq \emptyset} \equiv \bigcap_{i\in I }  \Pair{l_i:\sigma_i}$ and 
$\Pair{l_i:\sigma_i \mid i\in \emptyset} \equiv \record{}$, where $\equiv$ is syntactic identity up to associativity and commutativity of $\inter$.

\begin{lem}\label{lem:derivedLeq}
~ \hfil
\begin{enumerate}
\item \label{lem:derivedLeq-a} $\Pair{l:\sigma}\inter\Pair{l:\tau} = \Pair{l:\sigma\inter\tau}$
\item \label{lem:derivedLeq-b} $\Pair{l_0:\sigma} + \Pair{l_j : \tau_{j} \mid j \in J } =  \Pair{ l_j : \tau_{j} \mid j \in J }$ if $0 \in J$,
\item \label{lem:derivedLeq-c} $\Pair{l_0:\sigma} + \Pair{l_j : \tau_{j} \mid j \in J } = \Pair{l_0:\sigma}  \inter \Pair{ l_j : \tau_{j} \mid j \in J }$
	if $0 \not\in J$
\end{enumerate}
\end{lem}

\begin{proof} 

(\ref{lem:derivedLeq-a})
By  \ref{def:typeInclusionRec-new}.\ref{leq-ax-3}
$\record{l:\sigma \inter \tau} \leq \Pair{l:\sigma}$ and $\record{l:\sigma \inter \tau} \leq \Pair{l:\sigma}$ which implies
$\Pair{l:\sigma\inter\tau} \leq \Pair{l:\sigma}\inter\Pair{l:\tau}$ by Definition \ref{def:typeInclusionInt}.

\end{proof}

\begin{lem}\label{lem:normal-recordTypes-new}
~\hfill
\begin{enumerate}
\item \label{lem:normal-recordTypes-a}
	$\Pair{ l_i : \sigma_{i} \mid i \in I } \leq \Pair{l_j : \tau_{j} \mid j \in J } \Iff J \subseteq I \And \forall j \in J.\;\sigma_j \leq \tau_j $,
\item \label{lem:normal-recordTypes-ab}
	$ \Pair{ l_i : \sigma_{i} \ \mid \ i \in I } \inter  \Pair{ l_j : \tau_{j} \mid j \in J } =
		\Pair{l_i : \sigma_{i},  l_j : \tau_{j}, l_k:\sigma_k\inter\tau_k \mid i\in I\setminus J, j\in J\setminus I, k \in I \cap J}$,
\item \label{lem:normal-recordTypes-b}
	$ \Pair{ l_i : \sigma_{i} \ \mid \ i \in I } +  \Pair{ l_j : \tau_{j} \mid j \in J } =
		\Pair{l_i : \sigma_{i},  l_j : \tau_{j} \mid i\in I\setminus J, j\in J}$.
\item \label{lem:normal-recordTypes-c}
	$\forall \rho \in \TTR .\; \exists \ \Pair{l_i:\sigma_i  \mid  i\in I}.~
		\rho = \Pair{l_i:\sigma_i \mid  i\in I} $.
\end{enumerate}
\end{lem}
 
\begin{proof} Through all this proof let $\rho_1 \equiv \Pair{ l_i : \sigma_{i} \mid i \in I }$ and $\rho_2 \equiv \Pair{l_j : \tau_{j} \mid j \in J }$.

\begin{enumerate}
%(\ref{lem:normal-recordTypes-a}) 

\item The only if part is proved by induction over the derivation of $\rho_1 \leq \rho_2$. If this equation is an instance of axiom \ref{def:typeInclusionRec-new}.\ref{leq-ax-1} then $J = \emptyset \subseteq I$ and $\forall j \in J.\;\sigma_j \leq \tau_j$ is vacuously true.

%\noindent
Axiom \ref{def:typeInclusionRec-new}.\ref{leq-ax-2} doesn't apply being the labels $l_i$ pairwise distinct. 

%\noindent
In case the derivation ends by rule \ref{def:typeInclusionRec-new}.\ref{leq-ax-3} we have $I = J = \Set{l}$ and $\sigma \leq \tau$ by the 
premise of the rule.

%\noindent
In case of the axiom instance $\record{l_1:\sigma} \inter \record{l_2:\tau} \leq \record{l_1:\sigma}$ we have
$J = \Set{l_1} \subseteq \Set{l_1, l_2} = I$ and obviously $\sigma=\sigma$. 

%\noindent
Finally in case of deriving $\rho_1 \leq (\rho_3 \inter \rho_4)$ from $\rho_1 \leq \rho_3$ and 
$\rho_1 \leq \rho_4$, where $\rho_2 \equiv \rho_3 \inter \rho_4$, we have that for some $J', J''$ such that $J = J' \cup J''$ it
is $\rho_3 \equiv \Pair{l_h : \tau_{h} \mid h \in J'}$ and $\rho_4 \equiv \Pair{l_k : \tau_{k} \mid k \in J''}$. By induction we know that
$J' \subseteq I$ and $\sigma_h \leq \tau_h$ for all $h\in J'$ and $J'' \subseteq I$ and $\sigma_k \leq \tau_k$ for all $k\in J''$. Therefore
$J = J' \cup J'' \subseteq I$ and $\sigma_j \leq \tau_j$ for all $j \in J$.


For the if part we reason by induction over the cardinality of $J$. If $|J| = 0$ then $\rho_2 \equiv \record{}$, hence either $I = \emptyset$, but
then $\rho_1 \equiv \record{}$; or $I \neq \emptyset$ so that
$\rho_1 \leq \Pair{l_i:\sigma_i} \leq \record{}$ for any $i \in I$, using axiom \ref{def:typeInclusionRec-new}.\ref{leq-ax-1}.
If $|J| > 0$ then let $j_0 \in J$ be any index: then $\rho_2 \equiv \Pair{l_j:\tau_j \mid j \in J\setminus \Set{j_0}} \inter \Pair{l_{j_0}:\tau_{j_0}}$.
Now by induction $\rho_1 \leq \Pair{l_j:\tau_j \mid j \in J\setminus \Set{j_0}}$; by hypothesis $\sigma_{j_0}\leq \tau_{j_0}$  so
that $\rho_1 \leq  \Pair{l_{j_0}:\sigma_{j_0}} \leq  \Pair{l_{j_0}:\tau_{j_0}}$ and we conclude being $\inter$ the meet w.r.t. $\leq$. 

%(\ref{lem:normal-recordTypes-ab}) 
\item
This is an immediate consequence of commutativity, associativity, idempotency of $\inter$ and of Lemma
\ref{lem:derivedLeq}.\ref{lem:derivedLeq-a}.

%(\ref{lem:normal-recordTypes-b}) 
\item
If $I = \emptyset$ then$\rho_1  = \record{}$ and the thesis follow by 
\ref{def:typeInclusionRec-new}.\ref{leq-ax-4}. Otherwise we have:
\[\begin{array}{llll}
\rho_1 + \rho_2 & = & \bigcap_{i\in I} (\record{l_i:\sigma_i} + \rho_2) &
	 \mbox{by repeated applications of \ref{def:typeInclusionRec-new}.\ref{leq-ax-6}} \\
& = & \bigcap_{i\in I} \Pair{l_i:\sigma_i , l_j: \tau_j\mid i \not \in J, j \in J} & 
	\mbox{by Lemma \ref{lem:derivedLeq}.\ref{lem:derivedLeq-b} and \ref{lem:derivedLeq}.\ref{lem:derivedLeq-c}} \\
& = & \Pair{l_i : \sigma_{i},  l_j : \tau_{j} \mid i\in I\setminus J, j\in J} & \mbox{by abbreviation definition.}
\end{array}\]
	
\item By induction over $\rho$. If $\rho = \record{}$ there is nothing to prove. 
	
	\noindent
	If $\rho \equiv \rho_1 \inter \rho_2$ then by induction 
	$\rho_1 = \Pair{l_i^1:\sigma_i^1 \mid i \in I_1}$ and
	$\rho_2 = \Pair{l_i^2:\sigma_i^2 \mid i \in I_2}$ so that the thesis follows by
	(\ref{lem:normal-recordTypes-ab}) above and %the fact that $=$ is a congruence w.r.t. $\inter$.
	Lemma \ref{lem:congruence}.\ref{lem:congruence-b}.
	
	\noindent
	Similarly if $\rho \equiv \rho_1 + \rho_2$ the thesis follows by induction using
	(\ref{lem:normal-recordTypes-b}) and %the fact that $=$ is a congruence w.r.t. $+$.
	Lemma \ref{lem:congruence}.\ref{lem:congruence-c}.
\end{enumerate}
\end{proof}



\newpage
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_document.tex"
%%% End:


==> gen-int.tex <==
%!TEX root = main_document.tex

\newcommand{\Succ}{\textsf{Succ}}
%\newcommand{\Even}{\textsf{even}}
%\newcommand{\Odd}{\textsf{odd}}

\newpage
\subsection{Generating types for Class and Mixin combinators}

Let us consider the simplified class example $C_1 \equiv \Y(\lambda \self. R_1)$ (by omitting the state or equivalently by considering
$C_1$ as an instantiated class) where
\[R_1 \equiv \record{l = 3, m = \self.l + 1} \]
Then we consider the unfoldings of $C_1$:
\[\begin{array}{lll}
C_1^{[0]} & = & C_1 \\ [2mm]
C_1^{[1]} & = & R_1\Subst{C_1^{[0]}}{s} = \record{l = 3, m = C_1.l + 1} \\ [2mm]
C_1^{[2]} & = & R_1\Subst{C_1^{[1]}}{s} = \record{l = 3, m = 3 + 1} 
\end{array}\]
which are enough to compute 
\[C_1.m \reduces \record{l = 3, m = C_1.l + 1}.l + 1 \reduces 3 + 1 \]
In parallel to the unfolding we can generate the approximants with the respective types:
\[\begin{array}{lllll}
R_1^{[0]} & = & \Omega & : & \rho_1^{[0]} = \omega\\ [2mm]
R_1^{[1]} & = & R_1\Subst{R_1^{[0]}}{s} = \record{l = 3, m = \Omega} & : & \rho_1^{[1]} = \record{l:\Int, m: \omega}\\ [2 mm]
R_1^{[2]} & = & R_1\Subst{R_1^{[1]}}{s} = \record{l = 3, m = 3 + 1} & : & \rho_1^{[2]} =\record{l:\Int, m: \Int}
\end{array}\]
which are such that
\[\self:  \rho_1^{[i]} \vdash R_1^{[i+1]} : \rho_1^{[i+1]} \]
Given some intersection type theory (to be adapted to the case with records) we get
\[\self:  \rho_1^{[i]} \vdash R_1 : \rho_1^{[i+1]}  \quad (i =0,1) \qquad \mbox{and hence} \qquad
	\vdash C_1 : \rho_1^{[2]} =\record{l:\Int, m: \Int}\]
Note that, since no method of $C_1$ ever returns a value of the same type as $C_1$ itself, this class definition is not truly recursive,
and the unfoldings reach a fixed point in two steps; indeed three approximants are enough, and so are their intersection types.  


\medskip
A better example is $C_2 \equiv \Y(\lambda \self. R_2)$ where
\[R_2 \equiv \record{l = 3, m = \self  \Override \record{l = \self.l + 1}} \]
Note that $C_2$ can result from the application of a mixin to $C_1$ for example. In this case we have the unfoldings:
\[\begin{array}{lll}
C_2^{[0]} & = & C_2 \\ [2mm]
C_2^{[1]} & = & R_2\Subst{C_2^{[0]}}{s} = \record{l = 3, m = C_2^{[0]}  \Override \record{l = C_2^{[0]}.l + 1}} \\ [2mm]
C_2^{[2]} & = & R_2\Subst{C_2^{[1]}}{s} = 
	\record{l = 3, m = C_2^{[1]}  \Override \record{l = C_2^{[1]}.l + 1}} \\ [2mm]
	& \cdots
\end{array}\]
that reach their fixed point only after infinitely many steps.

The effect of the unfoldings is better viewed by looking at the respective approximants and types:
\[\begin{array}{lllll}
R_2^{[0]} & = & \Omega & : & \rho_2^{[0]} = \omega\\ [2mm]
R_2^{[1]} & = &  \record{l = 3, m = \Omega} & : & \rho_2^{[1]} = \record{l:\Int, m: \omega}\\ [2 mm]
R_2^{[2]} & = &  \record{l = 3, m = \record{l = 4, m = \Omega}} & : & \rho_2^{[2]} =\record{l:\Int, m: \record{l:\Int, m: \omega}} \\ [2mm]
	& \cdots
\end{array}\]
where $R_2^{[i+1]} = R_2\Subst{R_2^{[i]}}{s}$ similarly to the first example. We see also that 
\[ \rho_2^{[i+1]} = \record{l:\Int, m: \record{l:\Int, m: \rho_2^{[i]} }} \]
In fact we can generate all the $ \rho_2^{[i]}$ from the recursive type
\[\rho_2 = \mu t. \record{l:\Int, m: \record{l:\Int, m: t}} \]
where $\rho_2^{[i]}$ is obtained by taking the $i$-time unfolding of $\rho_2$ and then replacing any subexpression of the
shape $\mu t. \cdots$ by $\omega$.

\medskip
The idea of using the unfolding of a recursive type instead of computing the approximants and then the respective 
types doesn't apply smoothly to the case of the first example. The only choice for the recursive type seems:
\[ \rho_1 = \mu t. \record{l:\Int, m: \Int} \]
But then we don't get $\rho_1^{[1]} = \record{l:\Int, m: \omega}$; rather we obtain directly (and trivially)
\[ \rho_1^{[2]} =\record{l:\Int, m: \Int} = \record{l:\Int, m: \Int}\Subst{\rho_1}{t}\]
On the other hand we have
\[\vdash \lambda \self. R_1 : \record{l:\Int, m: \Int} \to  \record{l:\Int, m: \Int} \qquad \mbox{but} 
\qquad \not\vdash \lambda \self. R_1 : \omega \to  \record{l:\Int, m: \Int} 
\]
Actually a better choice is to prove
\[\vdash \lambda \self. R_1 : \omega \to  \record{l:\Int} \qquad \mbox{and} 
\qquad \vdash \lambda \self. R_1 : \record{l:\Int} \to  \record{l:\Int, m: \Int} 
\]
but the type $ \record{l:\Int}$ is hardly obtainable from $\rho_1$ in a uniform way.


\medskip
A further difficulty arises if we consider a more substantial use of intersection types, as with semantic types. Suppose that
we have the typings 
\[\vdash \underline{2k}:\Even, \quad \vdash \underline{2k+1}:\Odd
\qquad \mbox{and} \qquad x: \Even \vdash x+1:\Odd, \quad x: \Odd \vdash x+1:\Even\]
where $\underline{2k}$ and $\underline{2k+1}$ are numerals. Then we obtain the following typings of the approximants of $C_2$:
\[\begin{array}{lllll}
R_2^{[0]} & = & \Omega & : & \tilde{\rho}_2^{[0]} = \omega\\ [2mm]
R_2^{[1]} & = &  \record{l = 3, m = \Omega} & : & \tilde{\rho}_2^{[1]} = \record{l:\Odd, m: \omega}\\ [2 mm]
R_2^{[2]} & = &  \record{l = 3, m = \record{l = 4, m = \Omega}} & : & \tilde{\rho}_2^{[2]} =\record{l:\Odd, m: \record{l:\Even, m: \omega}} \\ [2mm]
	& \cdots
\end{array}\]
This typing is interesting since we have that 
\[ \vdash C_2 : \tilde{\rho}_2^{[n]} \qquad \mbox{for all $n$} \]
where
\[ \tilde{\rho}_2^{[n]}  = \record{l:\Odd, \underbrace{m: \langle l: Even, m: \langle \cdots  \,
	m}_{n} : \langle l:\sigma, m:\omega \rangle\, \cdots \rangle \rangle}
\]
with $\sigma = \Even$ if $n$ is odd, $\sigma = \Odd$ if $n$ is even. 

To generate the types $\tilde{\rho}_2^{[n]}$ from a recursive type consider:
\[\begin{array}{lllll}
\pi^{[0]} & = & o^{[0]} \quad = \quad \omega \\
\pi^{[n+1]} & = & \record{l:\Even, m: o^{[n]} } \\
o^{[n+1]} & = & \record{l:\Odd, m: \pi^{[n]} }
\end{array}\]
Then $\tilde{\rho}_2^{[n]} = o^{[n]}$. Now if we take
\[ \tilde{\rho}_2 = o = \mu t. \record{l:\Odd, m: \record{l: \Even, m: t}}\]
by repeatedly unfolding $o$ and replacing recursive type expressions by $\omega$ we get all the $\tilde{\rho}_2^{[2n]} = o^{[2n]}$ but not
the $\tilde{\rho}_2^{[2n+1]} = o^{[2n+1]}$.

A better idea seems to take
\[\pi = \mu t. \record{l:\Even, m: \record{l:\Odd, m: t } } \qquad \mbox{and} \qquad
	\tilde{\rho}_2 = \record{l:\Odd, m: \pi} \]
$\ldots$


\newpage
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_document.tex"
%%% End:

